Accelerated Runtime Verification of LTL Specifications with Counting Semantics

Runtime verification is an effective automated method for specification-based offline testing and analysis as well as online monitoring of complex systems. The specification language is often a variant of regular expressions or a popular temporal logic, such as LTL. This paper presents a novel and efficient parallel algorithm for verifying a more expressive version of LTL specifications that incorporates counting semantics, where nested quantifiers can be subject to numerical constraints. Such constraints are useful in evaluating thresholds (e.g., expected uptime of a web server). The significance of this extension is that it enables us to reason about the correctness of a large class of systems, such as web servers, OS kernels, and network behavior, where properties are required to be instantiated for parameterized requests, kernel objects, network nodes, etc. Our algorithm uses the popular {\em MapReduce} architecture to split a program trace into variable-based clusters at run time. Each cluster is then mapped to its respective monitor instances, verified, and reduced collectively on a multi-core CPU or the GPU. Our algorithm is fully implemented and we report very encouraging experimental results, where the monitoring overhead is negligible on real-world data sets.

==> background.tex <==
%!TEX root = main.tex
\section{Background}
\label{sec:bg}

\subsection{Linear Temporal Logic (LTL)}

%{\em Linear temporal logic} (\LTL) is a modal temporal logic used to encode 
%formulas about the future of a path.
Let $\AP$ be a finite set of {\em atomic propositions} and $\Sigma = 2^{\AP}$ a 
finite {\em alphabet}. A {\em trace} is a finite or infinite sequence of 
letters $w=a_0a_1\dots$, where for all $i \geq 0$, we have $a_i \in \Sigma$. We 
denote the set of all finite traces by $\Sigma^*$ and the set of all infinite 
traces by $\Sigma^\omega$. For a finite trace $u$ and a trace $w$, we write 
$uw$ to denote their {\em concatenation}.

\begin{definition}[LTL Syntax]
\LTL formulas are defined using the following grammar:
$$\varphi ::= \top \;\mid\; p \; \mid \; \neg\varphi \;\mid\; 
\varphi_1\vee\varphi_2 \; \mid \; \X\varphi \; \mid \; \varphi_1 \U \varphi_2$$

\noindent where $p \in \Sigma$, and, $\X$ (next) and $\U$ (until) are temporal operators.\qed
\end{definition}

\begin{definition}[\LTL Semantics] Let $w$ be an infinite trace in $\Sigma^w$, 
$i \geq 0$, and $\models$ denote the {\em 
satisfaction} relation. The semantics of \LTL is defined as follows:

\begin{tabbing}
\= $w, i \models \top$\\
\> $w, i \models p$ \hspace*{1cm} \= iff \hspace*{.5cm} \= $p \in a_i$ \\
\> $w, i \models \neg \varphi$ \> iff \> $w,i \not \models \varphi$ \\
\> $w, i \models \varphi_1\vee\varphi_2$ \> iff \> $w,i \models \varphi_1 \; \vee \; w, i \models \varphi_2$ \\
\> $w, i \models \X \varphi$ \> iff \> $w, i+1 \models \varphi$ \\
\> $w, i \models \varphi_1 \, \U \, \varphi_2$  \> iff \\
\> \hspace{1cm}$\exists k \geq i : w, k \models \varphi_2 \; \wedge \; \forall 
j: i \leq j < k: w, j \models \varphi_1$.
\end{tabbing}

\noindent Also, $w \models \varphi$ holds \; iff \; $w, 0 \models \varphi$ holds.\qed
\end{definition}
%The formula ($\X \varphi$), which uses the {\em next} temporal operator, 
%indicates that the formula is satisfied only when $\varphi$ holds in the {\em 
%next} state. The formula ($\varphi_1 \, \U \, \varphi_2$), which uses the {\em 
%until} temporal operator, indicates that the formula is satisfied only when 
%$\varphi_1$ continues to hold {\em until} $\varphi_2$ holds.
For example, in a multi-threaded system, correct thread initialization (i.e., a 
thread cannot be 
spawned unless it is initialized) can be captured by the \LTL property $\varphi 
\equiv (\exprop)$.

An \LTL formula $\varphi$ defines a set of traces, called a {\em property}, 
that satisfies the semantics of that formula. Throughout the paper, we use the 
terms `formula' and `property' interchangeably. We introduce abbreviation 
temporal operators: $\F \varphi$ ({\em finally} $\varphi$) denotes $\tru \, 
\U \, \varphi$, and $\G \varphi$ ({\em globally} $\varphi$) denotes $\neg \F 
\neg\varphi$. For instance, the {\em request-response} property $\G(p 
\Rightarrow \F 
q)$ means that `it is always the case that if proposition $p$ holds, then 
eventually proposition $q$ holds'.

\LTL is commonly used to verify a program against a certain property. We assume 
that a {\em program} is defined as a set $p$ of infinite traces. Normally, each 
program trace is a sequence of states that satisfies 
certain propositions, where each state is a valuation of 
program variables. We say that $p$ satisfies an \LTL property 
$\varphi$ (denoted $p \models \varphi$) \; iff \; for each each trace $w \in 
p$, we have $w \models \varphi$.

\subsection{3-valued Linear Temporal Logic (\LTLtri)}

Verifying \LTL properties at runtime boils down to the following problem: given 
the current program {\em finite} trace $w=a_0a_1a_2\dots a_n$, whether or 
not $\sigma$ belongs to a set of words defined by some property $\varphi$. 
However, \LTL semantics is defined over infinite traces and a running 
program can only deliver only a finite trace at run time. For example, given a 
finite trace $w = a_0a_1 \dots a_n$, it may be impossible for an observer 
(e.g., a runtime {\em monitor}) to decide weather the property $\F p$ is 
satisfied.

In~\cite{bls11}, the authors introduce 3-valued \LTL, where `$\tru$' denotes 
that the property is satisfied, `$\fals$' denotes that the property is 
violated, and `?' (the third value) denotes an unknown verdict, which means 
that given the current finite trace, it is impossible to determine whether the 
property is satisfied or violated.

\begin{definition}[\LTLtri semantics]
\label{def:ltl3}
Let $ u \in \Sigma^{*}$ be a finite word. The truth value of an \LTLtri formula 
$\varphi$ with respect to $u$, denoted by $[u \models \varphi]$, is defined as 
follows:

\begin{equation*}
	\left[ u \models \varphi \right] = 
		\begin{cases} \top & \text{if } \forall w \in \Sigma^\omega : u \cdot w \models \varphi,\\
		\bot & \text{if } \forall w \in \Sigma^\omega : u \cdot w \not \models \varphi,\\
		? & \text{otherwise}.~\blacksquare
	\end{cases}
\end{equation*}

\end{definition} 

Note that the syntax $\left[u \models \varphi \right]$ for \LTLtri semantics is 
defined over finite words as opposed to $u \models \varphi$ for \LTL semantics, 
which is defined over infinite words. For example, if proposition $p$ holds 
in some state of a finite trace, then property $\varphi=\mathbf{F}p$ holds for 
that trace. Otherwise, the valuation of $\varphi$ is `?', as it is unknown 
% whether $p$ will be encountered in the future or not. Similarly, the property 
% $\varphi=\mathbf{G}p$ will only be violated when the trace contains the 
% proposition $\neg p$, which violates the property. Otherwise, the verdict is `?' 
% since it is unknown if $\neg p$ will appear in the future or not.

\begin{definition} [Good, Bad, Ugly Prefixes] 
Given a language $L\subseteq\Sigma^{\omega}$ of infinite words over $\Sigma$, we 
call a finite word $u \in \Sigma^{*}$

\begin{itemize}
\item a \emph{good prefix} for $L$, if $\forall w \in \Sigma^{\omega} : u \cdot 
w \in L$ 
\item a \emph{bad prefix} for $L$, if $\forall w \in \Sigma^{\omega} : u \cdot w 
\notin L$ 
\item an \emph{ugly} prefix otherwise.\qed
\end{itemize}
\end{definition}

In \cite{bls11}, the authors introduce a stepwise method that takes as input an 
\LTLtri property $\varphi$ and synthesizes a deterministic finite state 
mashine (FSM) as a monitor that declares one of the values $\tru$, $\fals$, or ? 
for each change of state of the program under inspection. Intuitively, 
simulating a finite word $u$ on this FSM reaches a state that illustrates the 
valuation of $[u \models \varphi]$.

\begin{definition} [Monitor]
\label{def:monitor}
Let $\varphi$ be an \LTLtri formula over alphabet $\alphabet$. The {\em monitor} 
$\monitor^{\varphi}$ of $\varphi$ is the unique FSM $(\Sigma, Q, q_0, \delta, 
\lambda)$, where $Q$ is a set of states, $q_0$ is the initial state, $\delta 
\subseteq Q \times \Sigma \times Q$ is the transition relation, and $\lambda$ 
is a function that maps each state in $Q$ to a value in $\{\top, \bot, ?\}$, 
such that:
\begin{equation*}
\left[u \models \varphi\right] = \lambda(\delta(q_0, u)).~\blacksquare
\end{equation*}
\end{definition}

\begin{figure}[t]
  \centering
    \includegraphics[scale=.8]{exprop.pdf}
    \caption{The monitor for property $\varphi \equiv (\exprop)$}
    \label{fig:monitor}
\end{figure}

For example, consider the property $\varphi \equiv (\exprop)$ (i.e., a thread is 
not spawned until it is initialized). The corresponding monitor is shown in 
Figure~\ref{fig:monitor}~\cite{bls11}. The proposition $\mathit{true}$ denotes 
the set $\AP$ of all propositions. We use the term a 
\emph{conclusive state} to refer to monitor states $q_{\top}$ and $q_{\bot}$; 
i.e., states where $\lambda(q) = \top$ and $\lambda(q) = \bot$, respectively. 
Other states are called an {\em inconclusive state}. A monitor 
$\monitor^\varphi$ is constructed in a way that it recognizes minimal good and 
bad prefixes of $L(\varphi)$. Hence, if $\monitor^\varphi$ reaches a conclusive 
state, it stays in this {\em trap} state. 
SB: changes in response to Reviewer2

\begin{definition} [Monitorable Property]
\label{def:monitorable}
An \LTLtri \linebreak property $\varphi$ is {\em monitorable} if $L(\varphi)$ 
has no ugly prefixes. We denote the set of all monitorable 
\LTLtri properties by \LTLmon.\qed
\end{definition}

In other words, a property is \emph{monitorable} if for every finite word, there 
still exists a (possibly) infinite continuation that will determine whether the 
property is violated or satisfied. For example, property $\G\F p$ is not 
monitorable. This is intuitively because to declare satisfaction of 
$\G\F p$ the monitor has to identify an infinite loop that 
visits a state labeled by $p$, which is, of course, not possible at run time. 

\subsection{Finite LTL~\cite{mp95}}
\label{def:fltl}

The semantics of \LTL is defined over infinite traces. Finite \LTL 
(\FLTL) allows us to reason about finite traces for verifying 
properties at run time. The syntax of \FLTL is identical to that of \LTL and 
the semantics are based on the truth values $\mathbb{B}_2=\{\tru,\fals\}$.

\begin{definition} [\FLTL semantics]
Let $\varphi$ and $\psi$ be \LTL properties, and $u = u_0u_1 \cdots u_{n-1}$ 
be a finite trace.

	\begin{align*}
\left[u \models_{\text{\normalfont F}} \X\, \varphi\right] &= 
\begin{cases}
	[u_1 \models_{\text{\normalfont F}} \varphi] & \text{\normalfont if } u_1 \neq \epsilon \\
	\fals & \text{\normalfont otherwise}
\end{cases}\\ \\
\left[u \models_{\text{\normalfont F}} \varphi \,\U\, \psi\right] &= 
\begin{cases}
		\tru & \exists k \in [0,n-1]: [u_k \models_{\text{\normalfont F}} \psi] = \tru \;\;\wedge \\
	&\forall l \in [0,k) : [u^l \models_{\text{\normalfont F}} \varphi] = \tru\\
	\fals & \text{\normalfont otherwise}
\end{cases}
\end{align*}
where $\epsilon$ is the empty trace. The semantics of \FLTL for atomic 
propositions and Boolean combinations are identical to that of \LTL. \qed
\end{definition}

\subsection{4-valued LTL (LTL4) ~\cite{bls10-jlc}}

\LTLfour is designed for runtime verification by producing more informative 
verdicts than \FLTL. The syntax of \FLTL is identical to \LTL. The semantics of 
\LTLfour is defined based on values $\mathbb{B}_4=\{\tru,\TT,\FT,\fals\}$ ({\em 
true}, {\em presumably true}, {\em presumably false}, and {\em false} 
respectively). The semantics of \LTLfour is defined based on the semantics \LTL 
and \FLTL.

\begin{definition} [\LTLfour semantics]
\label{def:ltlfour}
Let $\varphi$ be an \LTLfour property and $u$ be a finite prefix of a trace.
\begin{equation*}
\left[u \models_4 \varphi\right] = 
\begin{cases}
	\tru & \forall v \in \alphabet^\omega : uv \models \varphi\\
	\fals & \forall v \in \alphabet^\omega: uv \not \models \varphi\\
	\TT & [u \models_F \varphi] \, \wedge \, \exists v \in 
\alphabet^\omega: uv \not \models \varphi \\
	\FT & [u \not \models_F \varphi] \, \wedge \, \exists v 
\in \alphabet^\omega: uv \models \varphi\qed
\end{cases}
\end{equation*}
\end{definition}
Thus, an \LTLfour property evaluates to $\tru$ with respect to a finite trace 
$u$, if the property remains {\em permanently satisfied}, meaning that for all 
possible infinite continuations of the trace, the property will always be 
satisfied in \LTL. Likewise, a valuation of $\fals$ means that the property will 
be {\em permanently violated}. If the property evaluates to $\TT$, this denotes 
that currently the property is satisfied yet there exists a continuation that 
could violate it. Finally, value $\FT$ denotes that currently the property is 
violated yet there exists a continuation that could satisfy it.

In \cite{bls10-jlc}, the authors introduce a method of synthesizing a 
{\em monitor}, as a deterministic finite state automaton, for an \LTLfour 
property.
\begin{definition} [Monitor]
\label{def:monitor2}
Let $\varphi$ be an \LTLfour formula over alphabet $\alphabet$. The {\em monitor} 
$\monitor^{\varphi}$ of $\varphi$ is the unique FSM $(\Sigma, Q, q_0, \delta, 
\lambda)$, where $Q$ is a set of states, $q_0$ is the initial state, $\delta 
\subseteq Q \times \Sigma \times Q$ is the transition relation, and $\lambda$ 
is a function that maps each state in $Q$ to a value in $\{\tru,\TT,\FT,\fals\}$, 
such that:
\begin{equation*}
\left[u \models \varphi\right] = \lambda(\delta(q_0, u)).~\blacksquare
\end{equation*}
\end{definition}
Thus, given an \LTLfour property $\varphi$ and a finite trace $u$, monitor 
$\monitor^{\varphi}$ is capable of producing a truth value in $\mathbb{B}_4$, 
which is equal to $[u \models_4 \varphi]$. For example, Figure~\ref{fig:ltl4} 
shows the monitor for property $\varphi = \G a \; \vee \; (b \, \U \, c)$. 
Observe that a monitor has two {\em trap} states 
(only an outgoing self loop), which map to 
truth values $\tru$ and $\fals$. They are trap states since these truth values 
imply permanent satisfaction (respectively, violation). Otherwise, states 
labeled by $\TT$ and $\FT$ can have outgoing transitions to other states.

\begin{figure}[h]
 \centering
  \includegraphics[width=0.6\columnwidth]{ltl4}
 \caption{\LTLfour monitor for property $\varphi = \G a \; \vee \; (b \, \U \, c)$.}
 \label{fig:ltl4}
\end{figure}
